The impact of observing cadence and undetected companions on the accuracy of planet mass measurements from radial velocity monitoring

We conduct experiments on both real and synthetic radial velocity (RV) data to quantify the impact that observing cadence, the number of RV observations, and undetected companions all have on the accuracy of small planet mass measurements. We run resampling experiments on four systems with small transiting planets and substantial public data from HIRES in order to explore how degrading observing cadence and the number of RVs affects the planets' mass measurement relative to a baseline value. From these experiments, we recommend that observers obtain 2--3 RVs per orbit of the inner-most planet and acquire at minimum 40 RVs. Following these guidelines, we then conduct simulations using synthetic RVs to explore the impact of undetected companions and untreated red noise on the masses of planets with known orbits. While undetected companions generally do not bias the masses of known planets, in some cases, when coupled with an inadequate observing baseline, they can cause the mass of an inner transiting planet to be systematically overestimated on average.

==> systemproperties.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 119130. System I %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Values from Luque et al. (2019) that are adopted by us
\newcommand{\logrhkI}{$-5.08 \pm 0.05$\xspace}
\newcommand{\mstarILXIX}{$1.00 \pm 0.03$\xspace}
\newcommand{\rstarILXIX}{$1.09 \pm 0.03$\xspace}
\newcommand{\periodIbLXIX}{$16.9841 \pm 0.0008$\xspace}
\newcommand{\tcIbLXIX}{$2458180.2842^{+0.0017}_{-0.0015}$\xspace}
\newcommand{\rpIb}{$2.63^{+0.11}_{-0.10}$\xspace}

\newcommand{\periodIb}{$16.9841 \pm 0.0008$\xspace}
\newcommand{\tcIb}{$2460232.8 \pm 0.9$\xspace}
\newcommand{\KIb}{$2.2 \pm 0.8$\xspace}
\newcommand{\mpIb}{$8.8 \pm 3.2$\xspace}
\newcommand{\mpIbupperlim}{$15.4$\xspace} % 98% confidence
\newcommand{\rhoIb}{$2.7 \pm 1.0$\xspace}
\newcommand{\periodIc}{$200.3 \pm 2.9$\xspace}
\newcommand{\tcIc}{$2460111.9 \pm 6.9$\xspace}
\newcommand{\KIc}{$4.9 \pm 1.2$\xspace}
\newcommand{\msiniIc}{$44.4 \pm 10.9$\xspace}

% Values from Luque et al. (2019) used for comparison
\newcommand{\mpIbLXIX}{$24.5 \pm 4.4$\xspace} % Mass measurement from Luque et al. (2019)
\newcommand{\rhoIbLXIX}{$7.4^{+1.6}_{-1.5}$\xspace} % Density from Luque et al. (2019)

\newcommand{\gammarvCARMENESI}{$-0.3 \pm 3.2$\xspace}
\newcommand{\sigmarvCARMENESI}{$4.8 \pm 1.4$\xspace}
\newcommand{\gammarvHARPSI}{$-0.7 \pm 1.0$\xspace}
\newcommand{\sigmarvHARPSI}{$2.7 \pm 0.8$\xspace}
\newcommand{\gammarvHARPSNI}{$1.4 \pm 1.0$\xspace}
\newcommand{\sigmarvHARPSNI}{$2.8 \pm 1.1$\xspace}
\newcommand{\gammarvHIRESI}{$-1.7 \pm 1.2$\xspace}
\newcommand{\sigmarvHIRESI}{$1.7 \pm 1.0$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% TOI-669. System II %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarII}{$0.90 \pm 0.06$\xspace}
\newcommand{\rstarII}{$0.99 \pm 0.04$\xspace}
\newcommand{\uOneII}{$0.88 \pm 0.43$\xspace}
% Rtol threshold exceeded for u_1, so the posterior might be skewed
\newcommand{\uTwoII}{$-0.18 \pm 0.41$\xspace}
\newcommand{\teffII}{$5600 \pm 110$\xspace}
\newcommand{\fehII}{$-0.06 \pm 0.09$\xspace}
\newcommand{\ageII}{$8.6 \pm 2.9$\xspace}

\newcommand{\periodIIb}{$3.94515 \pm 0.00002$\xspace}
\newcommand{\tcBTJDIIb}{$1913.041 \pm 0.002$\xspace}
\newcommand{\rorIIb}{$0.024 \pm 0.001$\xspace}
% Rtol threshold exceeded for b_b, so the posterior might be skewed
\newcommand{\bIIb}{$0.23 \pm 0.18$\xspace}
% Upper limit for ecc_b represents 98% confidence.
\newcommand{\eccIIb}{$< 0.23$\xspace}
\newcommand{\omegafoldeddegIIb}{$196.2 \pm 64.3$\xspace}
\newcommand{\KIIb}{$4.30 \pm 0.62$\xspace}
\newcommand{\aorIIb}{$10.3 \pm 0.5$\xspace}
\newcommand{\aIIb}{$0.047 \pm 0.001$\xspace}
% Rtol threshold exceeded for rp_b, so the posterior might be skewed
\newcommand{\rpIIb}{$2.60 \pm 0.17$\xspace}
\newcommand{\mpIIb}{$9.8 \pm 1.5$\xspace}
% Rtol threshold exceeded for rho_b, so the posterior might be skewed
\newcommand{\rhoIIb}{$3.0 \pm 0.7$\xspace}
\newcommand{\teqIIb}{$1235 \pm 37$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincIIb}{$388.2 \pm 47.1$\xspace}
% Rtol threshold exceeded for dur_hr_b, so the posterior might be skewed
\newcommand{\durhrIIb}{$2.9 \pm 0.1$\xspace}
% Rtol threshold exceeded for tsm_b, so the posterior might be skewed
\newcommand{\tsmIIb}{$35 \pm 8$\xspace}
\newcommand{\inclIIb}{$88.7 \pm 1.0\degree$\xspace}

\newcommand{\meanfluxII}{$0.02 \pm 0.01$\xspace}
% Rtol threshold exceeded for sigma_phot, so the posterior might be skewed
\newcommand{\sigmaphotII}{$0.02 \pm 0.02$\xspace}
\newcommand{\gammarvHIRESII}{$-2.25 \pm 0.43$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESII}{$2.88 \pm 0.36$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HIP 8152. System III %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mstarIII}{$0.91 \pm 0.06$\xspace}
\newcommand{\rstarIII}{$0.95 \pm 0.04$\xspace}
% Rtol threshold exceeded for u_0, so the posterior might be skewed
\newcommand{\uOneIII}{$0.46 \pm 0.37$\xspace}
% Rtol threshold exceeded for u_1, so the posterior might be skewed
\newcommand{\uTwoIII}{$0.09 \pm 0.39$\xspace}
\newcommand{\teffIII}{$5530 \pm 110$\xspace}
\newcommand{\fehIII}{$-0.09 \pm 0.09$\xspace}
\newcommand{\ageIII}{$8.2 \pm 3.1$\xspace}

\newcommand{\periodIIIb}{$10.75101 \pm 0.00006$\xspace}
% Rtol threshold exceeded for period_c, so the posterior might be skewed
\newcommand{\periodIIIc}{$19.6053 \pm 0.0003$\xspace}
% Rtol threshold exceeded for t0_BTJD_b, so the posterior might be skewed
\newcommand{\tcBTJDIIIb}{$1758.620 \pm 0.002$\xspace}
\newcommand{\tcBTJDIIIc}{$1751.195 \pm 0.005$\xspace}
\newcommand{\rorIIIb}{$0.025 \pm 0.001$\xspace}
\newcommand{\rorIIIc}{$0.024 \pm 0.001$\xspace}
% Rtol threshold exceeded for b_b, so the posterior might be skewed
\newcommand{\bIIIb}{$0.67 \pm 0.07$\xspace}
% Rtol threshold exceeded for b_c, so the posterior might be skewed
\newcommand{\bIIIc}{$0.35 \pm 0.19$\xspace}
% Upper limit for ecc_b represents 98% confidence.
\newcommand{\eccIIIb}{$< 0.14$\xspace}
% Upper limit for ecc_c represents 98% confidence.
\newcommand{\eccIIIc}{$< 0.28$\xspace}
% Rtol threshold exceeded for omega_folded_deg_b, so the posterior might be skewed
\newcommand{\omegafoldeddegIIIb}{$161.8 \pm 137.1$\xspace}
% Rtol threshold exceeded for omega_folded_deg_c, so the posterior might be skewed
\newcommand{\omegafoldeddegIIIc}{$153.1 \pm 83.2$\xspace}
\newcommand{\KIIIb}{$2.42 \pm 0.53$\xspace}
\newcommand{\KIIIc}{$2.40 \pm 0.55$\xspace}
\newcommand{\aorIIIb}{$20.9 \pm 1.0$\xspace}
\newcommand{\aorIIIc}{$31.2 \pm 1.5$\xspace}
\newcommand{\aIIIb}{$0.092 \pm 0.002$\xspace}
\newcommand{\aIIIc}{$0.138 \pm 0.003$\xspace}
\newcommand{\rpIIIb}{$2.56 \pm 0.19$\xspace}
% Rtol threshold exceeded for rp_c, so the posterior might be skewed
\newcommand{\rpIIIc}{$2.48 \pm 0.19$\xspace}
\newcommand{\mpIIIb}{$7.8 \pm 1.8$\xspace}
\newcommand{\mpIIIc}{$9.4 \pm 2.2$\xspace}
% Rtol threshold exceeded for rho_b, so the posterior might be skewed
\newcommand{\rhoIIIb}{$2.5 \pm 0.8$\xspace}
% Rtol threshold exceeded for rho_c, so the posterior might be skewed
\newcommand{\rhoIIIc}{$3.4 \pm 1.1$\xspace}
\newcommand{\teqIIIb}{$855 \pm 28$\xspace}
\newcommand{\teqIIIc}{$699 \pm 23$\xspace}
% Rtol threshold exceeded for sinc_b, so the posterior might be skewed
\newcommand{\sincIIIb}{$88.9 \pm 11.6$\xspace}
% Rtol threshold exceeded for sinc_c, so the posterior might be skewed
\newcommand{\sincIIIc}{$39.9 \pm 5.2$\xspace}
% Rtol threshold exceeded for dur_hr_b, so the posterior might be skewed
\newcommand{\durhrIIIb}{$2.9 \pm 0.1$\xspace}
% Rtol threshold exceeded for dur_hr_c, so the posterior might be skewed
\newcommand{\durhrIIIc}{$4.3 \pm 0.3$\xspace}
% Rtol threshold exceeded for tsm_b, so the posterior might be skewed
\newcommand{\tsmIIIb}{$44 \pm 14$\xspace}
% Rtol threshold exceeded for tsm_c, so the posterior might be skewed
\newcommand{\tsmIIIc}{$27 \pm 9$\xspace}
% Rtol threshold exceeded for inc_b, so the posterior might be skewed
\newcommand{\inclIIIb}{$88.2 \pm 0.2$\xspace}
% Rtol threshold exceeded for inc_c, so the posterior might be skewed
\newcommand{\inclIIIc}{$89.3 \pm 0.4$\xspace}

\newcommand{\meanfluxIII}{$0.009 \pm 0.006$\xspace}
% Rtol threshold exceeded for sigma_phot, so the posterior might be skewed
\newcommand{\sigmaphotIII}{$0.01 \pm 0.01$\xspace}
\newcommand{\gammarvHIRESIII}{$-1.44 \pm 0.37$\xspace}
% Rtol threshold exceeded for sigma_rv_HIRES, so the posterior might be skewed
\newcommand{\sigmarvHIRESIII}{$3.15 \pm 0.30$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% TOI-1444. System IV %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% These values come from Dai et al. (2021)
\newcommand{\rpIVb}{$1.40 \pm 0.06$\xspace}
\newcommand{\mpIVb}{$3.9 \pm 0.7$\xspace}
\newcommand{\mpIVc}{$11.8 \pm 2.9$\xspace} % msini

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% TOI-1272. System V  %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% These values come from MacDougall et al. (2022)
\newcommand{\rpVb}{$4.14 \pm 0.21$\xspace}
\newcommand{\eVb}{$0.34 \pm 0.06$\xspace}
\newcommand{\mpVb}{$24.6 \pm 2.3$\xspace}
\newcommand{\mpVc}{$26.7 \pm 3.1$\xspace} % msini

